Greenformers: Improving Computation and Memory Efficiency in Transformer Models via Low-Rank Approximation

In this thesis, we introduce Greenformers, a collection of model efficiency methods to improve the model efficiency of the recently renowned transformer models with a low-rank approximation approach. The development trend of deep learning models tends to results in a more complex and larger model. Although it leads to a better and more accurate prediction, the resulting model becomes even more costly, as it requires weeks of training with a huge amount of GPU resources. Particularly, the size and computational cost of transformer-based models have increased tremendously since its first debut in 2017 from ~100 million parameters up to ~1.6 trillion parameters in early 2021. This computationally hungry model also incurs a substantial cost to the environment and even reaches an alarming level of carbon footprint. Some of these models are so massive that it is even impossible to run the model without a GPU cluster. Greenformers improve the model efficiency of transformer models by applying low-rank approximation approaches. Specifically, we propose a low-rank factorization approach to improve the efficiency of the transformer model called Low-Rank Transformer. We further compare our model with an existing low-rank factorization approach called Linformer. Based on our analysis, the Low-Rank Transformer model is suitable for improving both the time and memory efficiency in processing short-sequence (<= 512) input data, while the Linformer model is suitable for improving the efficiency in processing long-sequence input data (>= 512). We also show that Low-Rank Transformer is more suitable for on-device deployment, as it significantly reduces the model size. Additionally, we estimate that applying LRT to the existing BERT-base model can significantly reduce the computational, economical, and environmental costs for developing such models by more than 30% of its original costs.

==> Makefile <==
thesis.pdf: main.tex \
				chapter/*.tex \

	latex main.tex
	bibtex main
	latex main.tex
	latex main.tex
	dvipdf main.dvi thesis.pdf

clean:
	rm *.aux *.bbl *.blg *.dvi *.pdf *.bak *.toc *.tol *.lof *.log *.lot
read:
	acroread thesis.pdf


==> chapter/old_but_gold/sec-1-introduction.tex <==
\chapter{Introduction}\label{sec-introduction}

\section{Motivation and Research Problems}

% Overview of the Motivation
Starting from AlexNet~\cite{krizhevsky2012alexnet} in 2012, deep learning models have made significant progression in various fields. Along with its remarkable adoption and growth, the computational cost required for developing a deep learning model also rises significantly at an unprecedented rate. From 2012 to 2018, the computational cost required is estimated to increase by 300,000x~\cite{schwartz2019green}. From 2018 onward, the development of NLP models has shown an even sharper trend. Starting with ELMo ~\cite{peters2018elmo} with ~100M parameters in 2018, followed by BERT ~\cite{devlin2019bert} with ~340M parameters and ~\cite{radford2019gpt2} with ~1.5B parameters in 2019. Recently, two other gigantic models have been released: 1) GPT3~\cite{brown2020gpt3} with ~175B parameters and 2) Switch Transformer~\cite{fedus2021switch} with ~1.6T parameters. This enormous model size requires a huge amount of computational cost. This computationally hungry model also incurs a substantial cost to the environment and even reaches an alarming level of carbon footprint ~\cite{strubell2019energy}. Some of these models are so massive that it is even impossible to run the model in real-time with a single GPU device.

Several responses have been made to address this problem and raise people's awareness to improve the efficiency of a deep learning model and reduce the overall carbon footprint. SustainNLP is a shared task ~\cite{wang2020sustainnlp} released with the goal of building energy-efficient solutions for the NLP model. Schwartz et al. ~\cite{schwartz2019green} explored a methodology to measure efficiency and introduce the term Green AI which refers to AI research that focuses on increasing computational efficiency. Dodge et al. (2019) ~\cite{dodge2019show} introduces a method for estimating the model performance as a function of computation cost. Strubell et al. (2019) analyzes the expected carbon footprint of NLP research and provide actionable suggestions to reduce computational costs and improve equity. Hernandez et al. (2020) ~\cite{hernandez2020measuring} shows the importance of both hardware and algorithmic efficiency in reducing the computational cost of developing a deep learning model and provide recommendations for reporting modeling efficiency in AI research. Recent benchmarks\cite{tay2021lra,wilie2020indonlu,cahyawijaya2021indonlg} are also considering the model efficiency as one of the metrics to compare the models listed on the benchmarks.

Different efforts have been done to improve the hardware and algorithm efficiency of developing a deep learning model. As shown in Table 2 in Hernandez et al. (2020) ~\cite{hernandez2020measuring}, 44x less computation cost is required to achieve the same level of performance as AlexNet. While the architectural shift from recurrent neural network models such as Seq2seq~\cite{ilya2014seq2seq} and GNMT~\cite{johnson2017googles} to transformer model~\cite{vaswani2017transformer} leads to an increase of computational efficiency by 61x and 9x respectively. All these improvements are made possible through numbers of efficiency methods such as distillation~\cite{hinton2015distil,zhang020ternarybert,sun2020mobilebert}, pruning~\cite{lecun1990obd,hasibi1993sodpruning,hao2016pruning,han2015learningprune,frankle2019lottery,xu2021networkpruning}, quantization~\cite{jacob2018quantization,zhang020ternarybert,bai2020binarybert}, fast adaptation ~\cite{finn2017maml, winata2020fa-casr, winata2020mtl}, data cleansing~\cite{lee2019denoise, kobayashi2020influence, bang2021fakenews}, distributed training~\cite{fairscale2021,rasley2020deepspeed,rajbhandari2020zero}, mixed-precision~\cite{micikevicius2018mixed}, and efficient model~\cite{shen2021efficientattn,dai2021mesm, winata2020lrt, winata2021mme,tan2020efficientnet,wang2020linformer,katharopoulos2020lineartrf,choromanski2021performer}.

% Overview of different solutions
\begin{table}[!t]
\centering
\resizebox{0.85\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \textbf{Require} & \textbf{Training} & \textbf{Fine-Tuning} & \textbf{Inference} \\
     & \textbf{Prior Model} & \textbf{Efficient} &  \textbf{Efficient} & \textbf{Efficient} \\
    \midrule
    Distillation & \cmark & \xmark & \cmark / \xmark & \cmark \\
    Pruning & \cmark & \xmark & \cmark / \xmark & \cmark \\
    Quantization & \cmark & \xmark & \xmark & \cmark \\
    Fast Adaptation & \xmark / \cmark & \xmark & \cmark & \xmark \\
    Data Cleansing & \xmark & \cmark & \cmark & \xmark \\
    Distributed Training & \xmark & \cmark & \cmark & \xmark \\
    Mixed-Precision & \xmark & \cmark & \cmark & \cmark \\
    Efficient Model & \xmark & \cmark & \cmark & \cmark \\  \bottomrule
    \end{tabular}
}
\caption{Comparison of different efficiency methods}
\label{tab:computing-efficiency}
\end{table}

As shown in Table \ref{tab:computing-efficiency}, depending on when it is applied, an efficiency method can provide different effect to the computational cost on different modeling phase. Distillation, pruning, and quantization can reduce the computational cost drastically during the inference phase, but these methods require having a prior model which make the overall training cost higher. For distillation and pruning, fine-tuning process could also become more efficient as the distillation and pruning can be applied beforehand. Mixed-precision and efficient model decrease the computational cost during both training, fine-tuning, and inference. Nevertheless applying mixed-precision during inference might produce a slight inconsistent prediction as a result of rounding error. Unlike the other approaches, fast adaptation, data cleansing, and distributed training do not reduce the  computational cost of the model, but these approaches can reduce the actual training time during the training and/or fine-tuning in different ways. Fast adaptation methods allow the model to learn a representation that can quickly adapt to a new task, hence resulting in a more efficient fine-tuning phase. Data cleansing makes training and fine-tuning phases more efficient by reducing the number of samples to be trained by the model. Recent development in distributed training \cite{fairscale2021, rasley2020deepspeed, rajbhandari2020zero} allows better resource allocation and distribution strategy which ends up with significant memory reduction and faster training time.

% Application of the solutions
In this thesis, we focus on improving the computational efficiency by constructing a more efficient variant for attention-based models. We conduct our experiments in two different modality settings: 1) audio-modality setting and 2) multimodal (text, video, and audio) setting. In audio-modality setting, we conduct experiment on speech recognition task where we utilize low-rank factorization to factorize the model parameters. With this approach, the model size and computational cost can be decreased significantly, yielding a more efficient speech recognition model. In multimodal setting, we conduct experiment on multimodal emotion recognition task and develop a novel sparse cross-modal attention mechanism. The sparse cross-modal attention mechanism learns to remove noisy features from the video and audio modalities by using the information from the text modality, producing a smaller and more robust feature set. We provide extensive analysis regarding the performance and efficiency trade-off of our proposed models and provide recommendations for the best rank and sparsity settings.

% Additional Points
Additionally, we explore the applicability on efficient attention-based model to genomics data. We conduct experiment on Alzheimer's disease risk prediction on Chinese cohort. In this task, given a genomics sequence, our goal is to predict the risk of the subject of getting Alzheimer's disease. We formulate this task as a long sequence prediction task with a sequence length of $\sim$30,000 long. We utilize an attention-based model with linear complexity and compare the result with the existing FDA approved risk scoring model and other deep learning variants.

\section{Thesis Outline}

The contents of this thesis are focused on application of efficient modeling technique for attention-based model in different modality settings. The rest of the thesis is divided into five chapters and organized as follows:

\begin{itemize}
    \item Chapter 2 (Preliminaries and Related Work) introduces the background and important related works on matrix factorization, sparse matrix computation, and attention-based model.
    \item  Chapter 3 (Low-Rank Transformer for Speech Recognition) presents matrix factorization method to reduce the storage and computational cost of an attention-based model in speech recognition task.
    \item  Chapter 4 (Sparse Cross-Modal Attention Mechanism for Multimodal Emotion Recognition) introdudes a sparse cross-modal-attention approach to reduce the computational cost of an attention-based model in multimodal emotion recognition task.
    % \item  Chapter 5 (Influence-based Cleansing for COVID-19 Fake News Detection) discusses a data cleansing method for reducing noisy data and reduce the overall training time.
    \item  Chapter 5 (Linear Attention for Alzheimer's Disease Risk Prediction) shows the application of efficient attention-based model on long genome understanding task for predicting Alzheimer's disease in Chinese cohort.
    \item Chapter 6 (Conclusion) summarizes this thesis and the significance of the efficient attention-based models, and discusses the possible future research directions.
\end{itemize}

\newpage

==> chapter/old_but_gold/sec-5-linformer.tex <==
\chapter{Low-Rank Attention Mechanism for Alzheimer's Disease Risk Prediction}
\label{sec-linear-attention}

% Problem statement of the bottleneck
Recent development in genome modeling shows that deep learning models, including attention-based variant, could achieve pretty impressive performance on multiple haploid regulatory elements prediction tasks in genomics outperforming the other models by a large margin \cite{zhou2015dsea,zaheer2020bigbird,ji2020dnabert,umarov2017cnnprom,umarov2019promidd,min2017denhancer,yin2019dhistone}. Extending this approach for phenotype prediction, such as disease risk prediction, might provide huge advantages from improving the prediction accuracy and creating a new set of analytical tools for better understanding the genomics interaction of a certain phenotype characteristic. In this chapter, we explore the possibility of applying efficient attention-based model on Alzheimer's disease risk prediction task using genomics sequence. Alzheimer's disease is one of the most devastating brain disorders in elderly. It is estimated that nearly 36 million are affected to Alzheimer's disease globally and the number is expected to reach 115 million by 2050 \cite{huynh2017ad}. Disease risk prediction for Alzheimer's disease can help to prolong the healthspan of an individual with potential Alzheimer's disease trait and enable research to get better understanding of the disease progression from a very early stage.

Compared to haploid regulatory elements prediction, genomic modeling for disease risk prediction requires the model to capture much larger scale of input sequence. In regulatory elements prediction, regions are usually short and indicated by a certain pattern that are located inside regions. For instance, promoter is about 100-1000 nts~\cite{karni2007promoter} long and is associated with core promoter motifs such as TATA-box and CAAT-box, and GC-box~\cite{blackwood1998enhancer,lundin1994gcbox}. While enhancer is about 50 - 1,500 nts long and is associated with GATA-box and E-box~\cite{blackwood1998enhancer,anderson1998gata,ogilvy2007gata}. On the other hand, disease risk prediction requires the model to capture the aberration within at less a single gene and the average gene length inside human genome is around 24,000 base pairs long \cite{fuchs2014gene-length}. This sequence will be even longer when we would like to consider for neighbouring regulatory elements such as promoter, and the remote regulatory elements such as enhancer and silencer, which could be located up to one million base pair away from the corresponding gene\cite{pennacchio2013enhancer}. Moreover, most animals genome, including human, are diploid. This will not only increase the size of the data but it also requires additional methods to encode and process the diploid information as the haploid sequences (haplotypes) of a diploid chromosome is not directly observable.

% Solutions to the problem
To tackle the aforementioned problems, we propose two solutions: 1) we extend SentencePiece tokenization to aggregate multiple nucleotides into a single token for different diploid sequence representations and 2) we apply a linear-attention mechanism to enable the attention-based model to capture even longer sequence. We show that SentencePiece tokenization can reduce the computational cost effectively by producing set of tokens constructed from several base pairs, that are not only reducing the length of the sequence but also maintaining the robustness of the token over shifting, extension, and mutation. We thus employs linear attention mechanism which allows the model to reduce the memory bottleneck from $O(n^2)$ to $O(n)$ space complexity which significantly increase the capacity of the model to process longer input sequence. These two approaches allow us to capture around 35x longer sequence from $\sim$1,000 nts long to $\sim$35,0000 sequence length.

For processing the diploid chromosome, we explore two different representations. Firstly, we introduce a diplotype token representation, where we encode a diploid chromosome sequence into 66 diplotype tokens comprising combination of 11 tokens which represents 4 nucleotide tokens (\texttt{A}, \texttt{G}, \texttt{T}, and \texttt{C}), unspecified token (\texttt{N}), and insertion-deletion tokens (\texttt{AI}, \texttt{GI}, \texttt{TI}, \texttt{CI}, \texttt{NI}, and \texttt{DEL}). Secondly, we perform phasing to estimate the two haplotypes, one from each parent, and encode the token with 5 types of haplotype token comprising adenine (\texttt{A}), guanine (\texttt{G}), thymine (\texttt{T}), and cytosine (\texttt{C}), and unspecified (\texttt{N}). Our experiment result suggests that linear attention-mechanism with diplotype token representation can effectively model long diplotype for disease prediction and can produce higher score compared to the Food and Drug Administration (FDA) approved feature set for predicting Alzheimer's disease and the model with estimated haplotypes as its input. We further analyze that our model can capture important single nucleotide polymorphisms (SNPs) which are located inside the gene and the regulatory region. Our analysis approach can be further utilized to provide an explainable analysis on linear attention-based model.

\section{Preliminaries}
\label{sec-preliminary}

% Sequencing mechanism
\subsubsection{Sequencing Technology}

\begin{table}[ht]
\centering
\resizebox{0.8\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \textbf{Avg Read} & \textbf{Error} & \textbf{Cost per} & \textbf{Begin} \\
     & \textbf{Length} & \textbf{Rate} & \textbf{Megabase} & \textbf{From (Year)}\\
    \midrule
    Sanger & 400 - 900$^1$ & <0.3\%$^1$ & \$500$^2$ & 1953 \\
    NGS & 75 - 700$^1$ & 0.1\% - 1\%$^1$ & \$0.07 - \$84.39$^2$ & 2005 \\
    TGS & 250 - 2.3M$^3$ & <5\%$^4$ & \$0.01$^5$ & 2010 \\ \bottomrule
    \end{tabular}
}
\caption[Comparison of sequencing technology in different era]{Comparison of sequencing technology in different era. $^1$Kchouk et al. (2017)~\cite{kchouk2017sequencing-gen}}. $^2$Gong et al. (2018)~\cite{gong2018value-genomics}. $^3$Amarasinghe et al. (2020)~\cite{amarasinghe2020tgs}. $^4$ Boluwatife A. Adewale (2020)~\cite{adewale2020will-tgs}. $^5$ Wetterstrand Kris A (2021)\cite{wetterstrand2021seq-cost}.
\label{tab:sequencing-comparison}.
\end{table}

According to National Institutes of Health (NIH), a genome is defined as ``An organism’s complete set of DNA, including all of the genes, makes up the genome. Each genome contains all of the information needed to build and maintain that organism''\cite{goldman2016genome}. This genome data can be retrieved from a cell via a technique called \textbf{sequencing}. Sequencing technique is first introduced in 1953 by Frederick Sanger\cite{giani2019genomics} and is commonly known as Sanger sequencing. Sanger sequencing opens the first generation sequencing era and since then sequencing technology has been rapidly growing to the era of next-gen sequencing (NGS) in 2005\cite{adewale2020will-tgs} and to the third generation sequencing (TGS) in 2010s\cite{giani2019genomics}. Different sequencing techniques have been developed during the NGS and TGS era, each with different characteristics of reading data ~\cite{kchouk2017sequencing-gen}. Table~\ref{tab:sequencing-comparison} shows a simplified view of the comparison of each sequencing technology on each era.

\subsubsection{Human Genome}

A human genome consists of 23 pairs of chromosomes, each chromosome comprises of tens to hundreds of millions of nucleotides long sequence. There are four different kind of nucleotides: adenine (\texttt{A}), guanine (\texttt{G}), thymine (\texttt{T}), and cytosine (\texttt{C}) each connected to its reverse complement, i.e., \texttt{A} with \texttt{T} and \texttt{C} with \texttt{G}, which construct a deoxyribonucleic acid (DNA). Some regions inside a chromosome encode the template for creating a protein sequence. These regions are called as genes. As human chromosomes are diploid (paired), there are also two copies of the same gene inside a human body. Each copy of a gene is called allele. 

In 1911, the terms ``phenotype'' and ``genotype'' are introduced\cite{johannsen1911genotype}. Phenotype refers to the physical or observable characteristic of an individual , while genotype refers to a genetic characteristic of an individual. As the definition of genotype is rather broad and fluid depending to the context, in this work, we use the term diploid genotype (diplotype) as the sequence of nucleotides from a paired chromosome and haploid genotype (haplotype) as the sequence of nucleotides from a single chromosome. Specifically, we define a haplotype as a sequence $H = (h_1, h_2, ..., h_n)$, where $h_i$ denotes the nucleotide corresponding to the position $i$ and a diplotype as a sequence $D = (d_1, d_2, ..., xd_n)$, where $d_i$ denotes the pair-nucleotide corresponding to the position $i$. As human genome consists of diploid chromosomes, information of a pair of nucleotide sequences can be represented in two different ways: 1) as a set of two haplotypes $S = {H_1, H_2}$ where $H1$ and $H2$ are the two haplotypes, one for each chromosome; or 2) as a diplotype which can be visualize as an assembly graph $G = (B, E)$, where $B$ is a set of nucleotide, and $E$ denotes the edge connecting each nucleotide. Figure~\ref{fig:sequence_representation} shows the example of each sequence representation.

\begin{figure}[ht]
    \centering
    \resizebox{1.0\textwidth}{!}{
        \includegraphics[scale=1.0]{images/chapter-5/haploid-diploid.pdf}
    }
    \caption[DNA sequence representation for haploid and diploid chromosome]{DNA sequence representation for haploid and diploid chromosome. (a) Haplotype representation of a haploid chromosome (b) Two haplotypes  representation of a diploid chromosome. (c) Diplotype representation of a diploid chromosome.}
    \label{fig:sequence_representation}
\end{figure}

Intuitively, for a diploid chromosome, two haplotypes representation would be the most biologically plausible way to representing a diploid  dchromosome sequence. Unfortunately, due to the nature of primer design in sequencing \cite{pham2021aspcr-hlac,darawi2013aspcr-ad}, these haplotypes cannot be directly observed with a standard sequencing technique. Nevertheless, the two haploid sequences can be approximated with a technique called \textbf{phasing}. 
% Further discussion on phasing is explained on Section \ref{sec-phasing}.

\subsubsection{Phasing}
\label{sec-phasing}

\begin{figure}[ht]
    \centering
    \resizebox{0.75\textwidth}{!}{
        \includegraphics[scale=1.0]{images/chapter-5/phasing.pdf}
    }
    \caption[Example of sequence phasing]{Example of sequence phasing. (a) Correctly phased haplotypes. (b) Ambiguous phased haplotypes which possibly produces a chimeric haplotype. R denotes the reference genome. G denotes the genotype of the diploid sequence. H1 and H2 denote the two haplotypes of the diploid sequence.}
    \label{fig:phasing}
\end{figure}

Phasing is a technique to estimate haplotypes from a diploid chromosome sequence. There are many different phasing techniques have been developed, each with different algorithm, input information, and supported sequencing technology\cite{browning2007beagle,browning2009beagle,patterson2014whatshap}. In general, phasing method finds the overlapping region from the aligned read data and split the sequence based on the variation. If there are more than one non-overlapping read region with variations, a probabilistic estimation is used to determine the most-likely variant for each haploid sequence. This often leads to the production of chimeric sequence where generated haplotypes are mixed from the  maternal and paternal alleles \cite{giani2019genomics}. This often becomes more severe when the read length and read coverage is low. Although this problem will likely be solved with the latest long-read sequencing technology of third-generation sequencing, but due to its limitations \cite{xiao2020tgs}, next-generation sequencing is still more favorable for current genomics analysis. The visualization correctly phased sequence and the potential chimeric sequence from phasing method are shown in Figure \ref{fig:phasing}.

\section{Methodology}

\subsection{Sequence Representation}
As shown in Figure~\ref{fig:sequence_representation}, we represent a diploid chromosome sequence in two ways: 1) set of two haplotypes representation and 2) diplotype representation. In the following section, we explain the encoding of each representation.

\subsubsection{Haplotype Token Encoding}

Haplotype sequence consists of four types of nucleotide, i.e, adenine (\texttt{A}), guanine (\texttt{G}), thymine (\texttt{T}), and cytosine (\texttt{C}). In the practical case, an additional nucleotide code \texttt{N} is used to represent an unspecified nucleotide at a certain position. Unspecified token can occur when there is no read data on a certain region and it is used in many bioinformatics application such as in the reference genome (RefSeq) \cite{pruitt2000refseq,pruitt2001refseq,maglott2000refseq,oleary2015refseq} which is used in many downstream analysis in genomics study. In this case, we define a vocabulary of haplotype token consisting of five tokens: adenine (\texttt{A}), guanine (\texttt{G}), thymine (\texttt{T}), cytosine (\texttt{C}), and unspecified (\texttt{N}) tokens.

\subsubsection{Diplotype Token Encoding}

\begin{figure}[!h]
    \centering
    \resizebox{0.9\textwidth}{!}{
        \includegraphics[scale=1.0]{images/chapter-5/mutation.pdf}
    }
    \caption[Mutation patterns in genomic sequence]{Mutation patterns in genomic sequence. R denotes a reference sequence and H denotes a haplotype compared to the reference.}
    \label{fig:mutation_pattern}
\end{figure}

To avoid forging chimeric sequences and further reduce the computational cost, we introduce a diplotype sequence representation. A diplotype token represents the combination of haplotype tokens including mutation patterns. As shown in Figure \ref{fig:mutation_pattern}, there are three mutation patterns that can occur on a genomic sequence, i.e., substitution, insertion, and deletion. A substitution mutation is commonly called as Single Nucleotide Polymorphism (SNP), while insertion and deletion are commonly called as \textbf{indel}. To accommodate all possible mutations, the diplotype token vocabulary is extended from the haplotype vocabulary in three steps. First, insertion and deletion patterns are introduced by extending the five tokens in the haplotype vocabulary (\texttt{A}, \texttt{T}, \texttt{C}, \texttt{G}, \texttt{N}) to 11 tokens (\texttt{A}, \texttt{T}, \texttt{C}, \texttt{G}, \texttt{N}, \texttt{DEL}, \texttt{AI}, \texttt{TI}, \texttt{CI}, \texttt{GI}, \texttt{NI}). \texttt{DEL} denotes deletion and \texttt{AI}, \texttt{TI}, \texttt{CI}, \texttt{GI}, and \texttt{NI} denote insertion that comes with the corresponding \texttt{A}, \texttt{T}, \texttt{C}, \texttt{G}, \texttt{N} tokens. Second, a combination of the 11 tokens are added, e.g., \texttt{A-T}, \texttt{C-A}, \texttt{G-T}, \texttt{A-TI}, \texttt{C-AI}, and \texttt{C-TI}; producing 66 tokens in total. Third, the diplotype tokens are mapped into a single character code to allow tokenization over a sequence of diplotype tokens. The complete map of diplotype tokens vocabulary is shown in Table \ref{tab:diplotype-tokens}.

\begin{CJK*}{UTF8}{gbsn}

\begin{table*}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lr|lr|lr|lr|lr|lr}
\toprule
\multicolumn{12}{c}{\textbf{Map of Diplotype Tokens}} \\ \midrule
\texttt{A} & \texttt{A} & \texttt{DEL-A} & 腌 & \texttt{A-C} & 嗄 & \texttt{AI-C} & 爸 & \texttt{C-G} & 嚓 & \texttt{CI-G} & 懂 \\
\texttt{C} & \texttt{C} & \texttt{DEL-AI} & 拔 & \texttt{A-G} & 阿 & \texttt{AI-CI} & 比 & \texttt{C-N} & 拆 & \texttt{CI-GI} & 答 \\
\texttt{G} & \texttt{G} & \texttt{DEL-C} & 吃 & \texttt{A-N} & 呵 & \texttt{AI-G} & 八 & \texttt{C-T} & 礤 & \texttt{CI-N} & 达 \\
\texttt{N} & \texttt{N} & \texttt{DEL-CI} & 搭 & \texttt{A-T} & 锕 & \texttt{AI-GI} & 霸 & \texttt{C-CI} & 车 & \texttt{CI-NI} & 第 \\
\texttt{T} & \texttt{T} & \texttt{DEL-G} & 想 & \texttt{A-AI} & 吖 & \texttt{AI-N} & 巴 & \texttt{C-GI} & 床 & \texttt{CI-T} & 瘩 \\
\texttt{AI} & \texttt{B} & \texttt{DEL-GI} & 香 & \texttt{A-CI} & 俺 & \texttt{AI-NI} & 逼 & \texttt{C-NI} & 穿 & \texttt{CI-TI} & 沓 \\
\texttt{CI} & \texttt{D} & \texttt{DEL-N} & 学 & \texttt{A-GI} & 安 & \texttt{AI-T} & 把 & \texttt{C-TI} & 出 & \texttt{G-GI} & 高 \\
\texttt{GI} & \texttt{H} & \texttt{DEL-NI} & 虚 & \texttt{A-NI} & 案 & \texttt{AI-TI} & 笔 & \texttt{GI-N} & \begin{CJK}{UTF8}{bkai}蝦\end{CJK} & \texttt{G-N} & 给 \\
\texttt{NI} & \texttt{O} & \texttt{DEL-T} & 徐 & \texttt{A-TI} & 按 & \texttt{N-NI} & 讷 & \texttt{GI-NI} & 合 & \texttt{G-NI} & 股 \\
\texttt{TI} & \texttt{U} & \texttt{DEL-TI} & 需 & \texttt{NI-T} & 喔 & \texttt{N-T} & 哪 & \texttt{GI-T} & 虾 & \texttt{G-T} & 个 \\
\texttt{DEL} & \texttt{X} & \texttt{T-TI} & 拓 & \texttt{NI-TI} & 侬 & \texttt{N-TI} & 娜 & \texttt{GI-TI} & 盒 & \texttt{G-TI} & 该 \\

\bottomrule
\end{tabular}
}
\caption{List of all diplotype tokens.} 
\label{tab:diplotype-tokens}
\end{table*}

\end{CJK*}

\subsection{Subword Tokenization}

Before feeding the sequence into the model, tokenization method such as k-mer tokenization~\cite{min2017kmeremb,ji2020dnabert} and gapped k-mer tokenization~\cite{ghandi2014gkmer,shrikumar2019gkmexplain} is commonly incorporated to enrich the token representation. In this work, we incorporate a subword tokenization method called SentencePiece\cite{kudo2018sentencepiece}. SentencePiece is a subword tokenization method that doesn't require any language-specific prior. SentencePiece enables the application of subword tokenization beyond NLP field. Internally, SentencePiece uses a slightly modified version of either Byte-pair-encoding (BPE), WordPiece, or Unigram subword tokenizations to generate the vocabulary and tokenize the sequence. Aside of the capability provided by the internal subword tokenization module, SentencePiece provides two additional pre-processing phases: 1) character normalization and 2) white-space preservation. In character normalization phase, SentencePiece transform a Unicode character into its semantically-equivalent decomposed-Unicode character following a certain normalization standard. In white-space preservation phase, SentencePiece escapes the \texttt{<space>} character into a meta symbol \_ (U+2581). The escaped sequence is then used as the input to the internal subword tokenization method for further processing. For our experiment, we utilize SentencePiece with NFCK\footnote{https://unicode.org/reports/tr15/} normalization standard and BPE tokenization for performing the subword tokenization.
 
\begin{figure}[!t]
    \centering
    \resizebox{0.75\textwidth}{!}{
        \includegraphics[scale=1.0]{images/chapter-5/subword.pdf}
    }
    \caption[SentencePiece with BPE subword tokenization]{SentencePiece with BPE subword tokenization. (a) Training phase. (b) Inference phase. The vocabulary is ordered by the frequency in descending order.}
    \label{fig:subword-tokenization}
\end{figure}

SentencePiece tokenization consists of two phases: training and inference. During the training phase, given a training data $\mathcal{D}$, SentencePiece tokenization builds a vocabulary with a dynamic length token representation. As SentencePiece supports several subword tokenization algorithms, the vocabulary generation process is slightly different from one to another. For BPE tokenization, the vocabulary is built bottom-up starting from single-length character and iteratively add longer character pairs based on the most-frequent pairs in $\mathcal{D}$. For WordPiece tokenization, the vocabulary is also built in bottom-up manner. But different to BPE tokenization, WordPiece scores character pairs by its likelihood in $\mathcal{D}$ instead of its frequency. Unlike BPE and WordPiece, Unigram method starts with a large combination of tokens and iteratively reduce the vocabulary size by reducing symbols with the least contribution to the loss of the Unigram language model build from $\mathcal{D}$ The training process of SentencePiece tokenization is stopped when it reaches a specified vocabulary size. From the training phase, SentencePiece tokenization produces a model file consisting the vocabulary and the rules to tokenize a sequence. During the inference phase, given a sequence data $\mathcal{S}$, SentencePiece tokenizes $\mathcal{S}$ into a set of tokens $(t_1, t_2, ..., t_n)$ according to the tokenization rules. Figure \ref{fig:subword-tokenization} shows the sample of the training and inference phase for the SentencePiece with BPE subword tokenization.

\subsection{Linear Attention via Low-Rank Approximation}
\label{sec-modeling}

\begin{figure}[h!]
\centering
\resizebox{1.0\linewidth}{!}{
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,841); %set diagram left start at 0, and has height of 841

%Rounded Rect [id:dp5714297523547804] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (46,229.6) .. controls (46,200) and (70,176) .. (99.6,176) -- (260.4,176) .. controls (290,176) and (314,200) .. (314,229.6) -- (314,406.92) .. controls (314,436.52) and (290,460.52) .. (260.4,460.52) -- (99.6,460.52) .. controls (70,460.52) and (46,436.52) .. (46,406.92) -- cycle ;
%Straight Lines [id:da6540714132752897] 
\draw    (63.57,531.01) -- (308.75,531.01) ;
%Straight Lines [id:da2552223576196192] 
\draw    (63.57,546.83) -- (308.75,546.83) ;
%Straight Lines [id:da5287245740026977] 
\draw    (72.02,530.7) -- (72.02,546.21) ;
%Straight Lines [id:da7802909319268548] 
\draw    (84.68,530.7) -- (84.68,546.21) ;
%Straight Lines [id:da009250469745178735] 
\draw    (97.35,530.7) -- (97.35,546.21) ;
%Straight Lines [id:da09657520654271445] 
\draw    (110.02,530.7) -- (110.02,546.21) ;
%Straight Lines [id:da2773047766319524] 
\draw    (122.68,530.7) -- (122.68,546.21) ;
%Straight Lines [id:da9469018780244521] 
\draw    (135.35,530.73) -- (135.35,546.24) ;
%Straight Lines [id:da8843576458323812] 
\draw    (148.02,530.73) -- (148.02,546.24) ;
%Straight Lines [id:da10708118621933205] 
\draw    (160.69,530.7) -- (160.69,546.21) ;
%Straight Lines [id:da10022361449132255] 
\draw    (173.35,530.7) -- (173.35,546.21) ;
%Straight Lines [id:da02044848950189182] 
\draw    (186.02,530.7) -- (186.02,546.21) ;
%Straight Lines [id:da34141043921192704] 
\draw    (198.69,530.7) -- (198.69,546.21) ;
%Straight Lines [id:da4350973326670483] 
\draw    (211.36,530.7) -- (211.36,546.21) ;
%Straight Lines [id:da8729347170566101] 
\draw    (224.02,530.73) -- (224.02,546.24) ;
%Straight Lines [id:da7140429918709219] 
\draw    (236.69,530.73) -- (236.69,546.24) ;
%Straight Lines [id:da18950754353288057] 
\draw    (249.36,531.32) -- (249.36,546.83) ;
%Straight Lines [id:da6595011861428421] 
\draw    (262.02,531.32) -- (262.02,546.83) ;
%Straight Lines [id:da9757734109443952] 
\draw    (274.69,531.32) -- (274.69,546.83) ;
%Straight Lines [id:da333244994325853] 
\draw    (287.36,531.35) -- (287.36,546.86) ;
%Straight Lines [id:da15097138382354514] 
\draw    (300.03,531.35) -- (300.03,546.86) ;
%Rounded Rect [id:dp817420116532737] 
\draw  [fill={rgb, 255:red, 255; green, 230; blue, 204 }  ,fill opacity=1 ] (71.2,477) .. controls (71.2,473.69) and (73.89,471) .. (77.2,471) -- (293.2,471) .. controls (296.51,471) and (299.2,473.69) .. (299.2,477) -- (299.2,495) .. controls (299.2,498.31) and (296.51,501) .. (293.2,501) -- (77.2,501) .. controls (73.89,501) and (71.2,498.31) .. (71.2,495) -- cycle ;
%Down Arrow [id:dp36060071820899864] 
\draw   (196.4,512.58) -- (191.05,512.58) -- (191.05,526.65) -- (180.36,526.65) -- (180.36,512.58) -- (175.02,512.58) -- (185.71,503.2) -- cycle ;
%Straight Lines [id:da32503879486933374] 
\draw    (186.35,470.73) -- (186.01,412.6) ;
\draw [shift={(186,410.6)}, rotate = 449.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6848116106430969] 
\draw    (235,436) -- (235,412) ;
\draw [shift={(235,410)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7788828366985489] 
\draw    (135,435.5) -- (135,412.5) ;
\draw [shift={(135,410.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp2918489107391051] 
\draw  [fill={rgb, 255:red, 248; green, 206; blue, 204 }  ,fill opacity=1 ] (100,365.23) .. controls (100,359.05) and (105.01,354.04) .. (111.19,354.04) -- (270.21,354.04) .. controls (276.39,354.04) and (281.4,359.05) .. (281.4,365.23) -- (281.4,398.81) .. controls (281.4,404.99) and (276.39,410) .. (270.21,410) -- (111.19,410) .. controls (105.01,410) and (100,404.99) .. (100,398.81) -- cycle ;
%Rounded Rect [id:dp2611062762947185] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (101,312) .. controls (101,308.69) and (103.69,306) .. (107,306) -- (276.4,306) .. controls (279.71,306) and (282.4,308.69) .. (282.4,312) -- (282.4,330) .. controls (282.4,333.31) and (279.71,336) .. (276.4,336) -- (107,336) .. controls (103.69,336) and (101,333.31) .. (101,330) -- cycle ;
%Rounded Rect [id:dp9104361053641665] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (101,204) .. controls (101,200.69) and (103.69,198) .. (107,198) -- (276.4,198) .. controls (279.71,198) and (282.4,200.69) .. (282.4,204) -- (282.4,222) .. controls (282.4,225.31) and (279.71,228) .. (276.4,228) -- (107,228) .. controls (103.69,228) and (101,225.31) .. (101,222) -- cycle ;
%Rounded Rect [id:dp4045675236487135] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (101,252) .. controls (101,248.69) and (103.69,246) .. (107,246) -- (276.4,246) .. controls (279.71,246) and (282.4,248.69) .. (282.4,252) -- (282.4,270) .. controls (282.4,273.31) and (279.71,276) .. (276.4,276) -- (107,276) .. controls (103.69,276) and (101,273.31) .. (101,270) -- cycle ;
%Straight Lines [id:da9458426825979824] 
\draw    (135,435.5) -- (235.67,435.83) ;
%Straight Lines [id:da25518520017580626] 
\draw    (185,335.67) -- (185.06,343.34) -- (185,354.33) ;
%Straight Lines [id:da40836889839865076] 
\draw    (186,306) -- (186,278) ;
\draw [shift={(186,276)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7818735959331948] 
\draw    (82,321.5) -- (99,321.5) ;
\draw [shift={(101,321.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da692256716637004] 
\draw    (82,321.5) -- (82,449.5) ;
%Straight Lines [id:da4425777779632257] 
\draw    (82,448.87) -- (186.4,449) ;
%Straight Lines [id:da23106696960822548] 
\draw    (185,227.67) -- (185.06,235.34) -- (185,246.33) ;
%Straight Lines [id:da6040624379633129] 
\draw    (82,213.5) -- (99,213.5) ;
\draw [shift={(101,213.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8657818206676262] 
\draw    (82,213.5) -- (82,295.5) ;
%Straight Lines [id:da23704046431368464] 
\draw    (82,294.87) -- (186.4,295) ;
%Straight Lines [id:da9043281586476462] 
\draw    (186,198) -- (186,158) ;
\draw [shift={(186,156)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp4906276456368184] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (71.2,132) .. controls (71.2,128.69) and (73.89,126) .. (77.2,126) -- (293.2,126) .. controls (296.51,126) and (299.2,128.69) .. (299.2,132) -- (299.2,150) .. controls (299.2,153.31) and (296.51,156) .. (293.2,156) -- (77.2,156) .. controls (73.89,156) and (71.2,153.31) .. (71.2,150) -- cycle ;
%Down Arrow [id:dp5710146831107652] 
\draw   (196.4,105.58) -- (191.05,105.58) -- (191.05,119.65) -- (180.36,119.65) -- (180.36,105.58) -- (175.02,105.58) -- (185.71,96.2) -- cycle ;
%Straight Lines [id:da3250756912664501] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (360.43,81.86) -- (361,568) ;
%Straight Lines [id:da317176949330536] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (723.43,79.86) -- (724,568) ;
%Straight Lines [id:da7069581741532798] 
\draw    (550.35,510.73) -- (550.02,474.6) ;
\draw [shift={(550,472.6)}, rotate = 449.47] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8253209039009313] 
\draw    (430,490.5) -- (430,434.5) ;
\draw [shift={(430,432.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4309264244502913] 
\draw    (430,490.5) -- (649.67,490.83) ;
%Rounded Rect [id:dp49584401220899776] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (374,404.94) .. controls (374,401.11) and (377.11,398) .. (380.94,398) -- (478.32,398) .. controls (482.15,398) and (485.26,401.11) .. (485.26,404.94) -- (485.26,425.76) .. controls (485.26,429.59) and (482.15,432.7) .. (478.32,432.7) -- (380.94,432.7) .. controls (377.11,432.7) and (374,429.59) .. (374,425.76) -- cycle ;
%Rounded Rect [id:dp9619742794419547] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (596,394.54) .. controls (596,389.27) and (600.27,385) .. (605.54,385) -- (697.72,385) .. controls (702.99,385) and (707.26,389.27) .. (707.26,394.54) -- (707.26,423.16) .. controls (707.26,428.42) and (702.99,432.7) .. (697.72,432.7) -- (605.54,432.7) .. controls (600.27,432.7) and (596,428.42) .. (596,423.16) -- cycle ;
%Rounded Rect [id:dp3793565799218024] 
\draw  [fill={rgb, 255:red, 255; green, 230; blue, 204 }  ,fill opacity=1 ] (495,521.54) .. controls (495,516.27) and (499.27,512) .. (504.54,512) -- (596.72,512) .. controls (601.99,512) and (606.26,516.27) .. (606.26,521.54) -- (606.26,550.16) .. controls (606.26,555.42) and (601.99,559.7) .. (596.72,559.7) -- (504.54,559.7) .. controls (499.27,559.7) and (495,555.42) .. (495,550.16) -- cycle ;
%Straight Lines [id:da3638431235739603] 
\draw    (650,490.5) -- (650,434.5) ;
\draw [shift={(650,432.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp23974078811329935] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (560.04,361.72) .. controls (563.87,361.72) and (566.98,364.82) .. (566.98,368.66) -- (566.98,466.04) .. controls (566.98,469.87) and (563.87,472.98) .. (560.04,472.98) -- (539.22,472.98) .. controls (535.39,472.98) and (532.28,469.87) .. (532.28,466.04) -- (532.28,368.66) .. controls (532.28,364.82) and (535.39,361.72) .. (539.22,361.72) -- cycle ;
%Straight Lines [id:da13555892800821556] 
\draw    (549.57,339.43) -- (549.5,361.5) ;
%Straight Lines [id:da7781358730959795] 
\draw    (429.57,339.43) -- (429.5,397.5) ;
%Shape: Output [id:dp4935714861564239] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (476.5,340.6) .. controls (476.5,333.97) and (481.65,328.6) .. (488,328.6) .. controls (494.35,328.6) and (499.5,333.97) .. (499.5,340.6) .. controls (499.5,347.23) and (494.35,352.6) .. (488,352.6) .. controls (481.65,352.6) and (476.5,347.23) .. (476.5,340.6) -- cycle (465,340.6) -- (476.5,340.6) (511,340.6) -- (499.5,340.6) ;
%Straight Lines [id:da3442374874589137] 
\draw    (429.5,340.6) -- (474.5,340.6) ;
\draw [shift={(476.5,340.6)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8733023931385413] 
\draw    (549.5,340.6) -- (501.5,340.6) ;
\draw [shift={(499.5,340.6)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9720202561348401] 
\draw    (488,328) -- (488,311) ;
\draw [shift={(488,309)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8070509425273988] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (433,231.01) .. controls (433,220.14) and (441.81,211.33) .. (452.67,211.33) -- (524.59,211.33) .. controls (535.45,211.33) and (544.26,220.14) .. (544.26,231.01) -- (544.26,290.02) .. controls (544.26,300.89) and (535.45,309.7) .. (524.59,309.7) -- (452.67,309.7) .. controls (441.81,309.7) and (433,300.89) .. (433,290.02) -- cycle ;
%Straight Lines [id:da08952465912412] 
\draw    (649.57,196.43) -- (649.5,385.5) ;
%Shape: Output [id:dp039211481171078644] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (546.5,197.6) .. controls (546.5,190.97) and (551.65,185.6) .. (558,185.6) .. controls (564.35,185.6) and (569.5,190.97) .. (569.5,197.6) .. controls (569.5,204.23) and (564.35,209.6) .. (558,209.6) .. controls (551.65,209.6) and (546.5,204.23) .. (546.5,197.6) -- cycle (535,197.6) -- (546.5,197.6) (581,197.6) -- (569.5,197.6) ;
%Straight Lines [id:da6607960102003837] 
\draw    (488.5,197.6) -- (544.5,197.6) ;
\draw [shift={(546.5,197.6)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8683403001978562] 
\draw    (649.5,197.6) -- (571.5,197.6) ;
\draw [shift={(569.5,197.6)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9989515012066065] 
\draw    (558,185) -- (558,167) ;
\draw [shift={(558,165)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp7983469739271837] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (503,126.54) .. controls (503,121.27) and (507.27,117) .. (512.54,117) -- (604.72,117) .. controls (609.99,117) and (614.26,121.27) .. (614.26,126.54) -- (614.26,155.16) .. controls (614.26,160.42) and (609.99,164.7) .. (604.72,164.7) -- (512.54,164.7) .. controls (507.27,164.7) and (503,160.42) .. (503,155.16) -- cycle ;
%Straight Lines [id:da35204360927755385] 
\draw    (488.5,197.6) -- (488.43,211.67) ;
%Straight Lines [id:da7871068518686761] 
\draw    (920.35,510.73) -- (920.02,474.6) ;
\draw [shift={(920,472.6)}, rotate = 449.47] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8758900234222797] 
\draw    (800,490.5) -- (800,434.5) ;
\draw [shift={(800,432.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7751336077284241] 
\draw    (800,490.5) -- (1019.67,490.83) ;
%Rounded Rect [id:dp838559039737457] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (744,404.94) .. controls (744,401.11) and (747.11,398) .. (750.94,398) -- (848.32,398) .. controls (852.15,398) and (855.26,401.11) .. (855.26,404.94) -- (855.26,425.76) .. controls (855.26,429.59) and (852.15,432.7) .. (848.32,432.7) -- (750.94,432.7) .. controls (747.11,432.7) and (744,429.59) .. (744,425.76) -- cycle ;
%Rounded Rect [id:dp5535312791762843] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (966,394.54) .. controls (966,389.27) and (970.27,385) .. (975.54,385) -- (1067.72,385) .. controls (1072.99,385) and (1077.26,389.27) .. (1077.26,394.54) -- (1077.26,423.16) .. controls (1077.26,428.42) and (1072.99,432.7) .. (1067.72,432.7) -- (975.54,432.7) .. controls (970.27,432.7) and (966,428.42) .. (966,423.16) -- cycle ;
%Rounded Rect [id:dp6440124577649587] 
\draw  [fill={rgb, 255:red, 255; green, 230; blue, 204 }  ,fill opacity=1 ] (865,521.54) .. controls (865,516.27) and (869.27,512) .. (874.54,512) -- (966.72,512) .. controls (971.99,512) and (976.26,516.27) .. (976.26,521.54) -- (976.26,550.16) .. controls (976.26,555.42) and (971.99,559.7) .. (966.72,559.7) -- (874.54,559.7) .. controls (869.27,559.7) and (865,555.42) .. (865,550.16) -- cycle ;
%Straight Lines [id:da3675978732075793] 
\draw    (1020,490.5) -- (1020,434.5) ;
\draw [shift={(1020,432.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8284274558426815] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (930.04,361.72) .. controls (933.87,361.72) and (936.98,364.82) .. (936.98,368.66) -- (936.98,466.04) .. controls (936.98,469.87) and (933.87,472.98) .. (930.04,472.98) -- (909.22,472.98) .. controls (905.39,472.98) and (902.28,469.87) .. (902.28,466.04) -- (902.28,368.66) .. controls (902.28,364.82) and (905.39,361.72) .. (909.22,361.72) -- cycle ;
%Straight Lines [id:da9202392699536629] 
\draw    (919.57,339.43) -- (919.5,361.5) ;
%Straight Lines [id:da2556168317704549] 
\draw    (799.57,339.43) -- (799.5,397.5) ;
%Shape: Output [id:dp8332392111294922] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (846.5,340.6) .. controls (846.5,333.97) and (851.65,328.6) .. (858,328.6) .. controls (864.35,328.6) and (869.5,333.97) .. (869.5,340.6) .. controls (869.5,347.23) and (864.35,352.6) .. (858,352.6) .. controls (851.65,352.6) and (846.5,347.23) .. (846.5,340.6) -- cycle (835,340.6) -- (846.5,340.6) (881,340.6) -- (869.5,340.6) ;
%Straight Lines [id:da844023694905402] 
\draw    (799.5,340.6) -- (844.5,340.6) ;
\draw [shift={(846.5,340.6)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9361322500315553] 
\draw    (919.5,340.6) -- (871.5,340.6) ;
\draw [shift={(869.5,340.6)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da05076665854215545] 
\draw    (858,328) -- (858,311) ;
\draw [shift={(858,309)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp6550264673795854] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (825,259.34) .. controls (825,252.52) and (830.52,247) .. (837.34,247) -- (877.66,247) .. controls (884.48,247) and (890,252.52) .. (890,259.34) -- (890,296.36) .. controls (890,303.17) and (884.48,308.7) .. (877.66,308.7) -- (837.34,308.7) .. controls (830.52,308.7) and (825,303.17) .. (825,296.36) -- cycle ;
%Straight Lines [id:da016285251418956537] 
\draw    (1019.57,196.43) -- (1019.5,385.5) ;
%Shape: Output [id:dp09943679963842955] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (916.5,197.6) .. controls (916.5,190.97) and (921.65,185.6) .. (928,185.6) .. controls (934.35,185.6) and (939.5,190.97) .. (939.5,197.6) .. controls (939.5,204.23) and (934.35,209.6) .. (928,209.6) .. controls (921.65,209.6) and (916.5,204.23) .. (916.5,197.6) -- cycle (905,197.6) -- (916.5,197.6) (951,197.6) -- (939.5,197.6) ;
%Straight Lines [id:da2371050756302978] 
\draw    (858.5,197.6) -- (914.5,197.6) ;
\draw [shift={(916.5,197.6)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7813903945634616] 
\draw    (1019.5,197.6) -- (941.5,197.6) ;
\draw [shift={(939.5,197.6)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da45536506005492017] 
\draw    (928,185) -- (928,167) ;
\draw [shift={(928,165)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp3890569864863834] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (873,126.54) .. controls (873,121.27) and (877.27,117) .. (882.54,117) -- (974.72,117) .. controls (979.99,117) and (984.26,121.27) .. (984.26,126.54) -- (984.26,155.16) .. controls (984.26,160.42) and (979.99,164.7) .. (974.72,164.7) -- (882.54,164.7) .. controls (877.27,164.7) and (873,160.42) .. (873,155.16) -- cycle ;
%Straight Lines [id:da2984386561611312] 
\draw    (858.5,197.6) -- (858.43,247.67) ;
%Flowchart: Alternative Process [id:dp5124788056804221] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (603.53,239.61) .. controls (603.53,233.62) and (608.38,228.76) .. (614.38,228.76) -- (780.68,228.76) .. controls (786.67,228.76) and (791.53,233.62) .. (791.53,239.61) -- (791.53,279.91) .. controls (791.53,285.91) and (786.67,290.76) .. (780.68,290.76) -- (614.38,290.76) .. controls (608.38,290.76) and (603.53,285.91) .. (603.53,279.91) -- cycle ;
%Straight Lines [id:da626957472675896] 
\draw    (544.01,273.5) -- (817.01,274.82)(543.99,276.5) -- (816.99,277.82) ;
\draw [shift={(825,276.36)}, rotate = 180.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp30007694177987954] 
\draw  [color={rgb, 255:red, 75; green, 172; blue, 162 }  ,draw opacity=1 ] (28,52) -- (1085.83,52) -- (1085.83,579.47) -- (28,579.47) -- cycle ;

% Text Node
\draw (73.69,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A};
% Text Node
\draw (86.36,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A};
% Text Node
\draw (99.03,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {G};
% Text Node
\draw (112.54,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {T};
% Text Node
\draw (124.36,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {C};
% Text Node
\draw (137.03,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {C};
% Text Node
\draw (150.54,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {T};
% Text Node
\draw (162.36,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {C};
% Text Node
\draw (175.88,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A};
% Text Node
\draw (187.84,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A};
% Text Node
\draw (200.37,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {T};
% Text Node
\draw (213.03,534.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {G};
% Text Node
\draw (226.54,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A};
% Text Node
\draw (238.37,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {C};
% Text Node
\draw (251.88,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {T};
% Text Node
\draw (263.98,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {T};
% Text Node
\draw (277.21,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A};
% Text Node
\draw (288.19,534.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {G};
% Text Node
\draw (54.52,526.7) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (305.05,526.7) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (152,477.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Embedding};
% Text Node
\draw (150,375.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Self Attention};
% Text Node
\draw (156,312.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Add \& Norm};
% Text Node
\draw (155,204.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Add \& Norm};
% Text Node
\draw (149,252.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Feed-Forward};
% Text Node
\draw (96,132.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Contextualized Embedding};
% Text Node
\draw (324,340) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{N×}};
% Text Node
\draw (496,494.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Input};
% Text Node
\draw (395,404.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{Q:n\times d_{k}}$};
% Text Node
\draw (518.93,344.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {$ $};
% Text Node
\draw (520,526.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{X:n\times d}$};
% Text Node
\draw (376,380.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Query};
% Text Node
\draw (518,343.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Key};
% Text Node
\draw (534,392.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{K^{T} :}$};
% Text Node
\draw (534,412.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \mathit{d_{k} \times n}$};
% Text Node
\draw (598,366.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Value};
% Text Node
\draw (619,399.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{V:n\times d_{v}}$};
% Text Node
\draw (477,327.6) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle \times $};
% Text Node
\draw (390,170.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Pairwise\\Similarities};
% Text Node
\draw (450,252.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{\rho (S):n\times n}$};
% Text Node
\draw (547,185.6) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle \times $};
% Text Node
\draw (504,99.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Output};
% Text Node
\draw (528,131.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{Y:n\times d_{v}}$};
% Text Node
\draw (866,494.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Input};
% Text Node
\draw (765,404.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{Q:n\times d_{k}}$};
% Text Node
\draw (888.93,344.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {$ $};
% Text Node
\draw (890,526.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{X:n\times d}$};
% Text Node
\draw (746,380.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Query};
% Text Node
\draw (888,343.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Key};
% Text Node
\draw (904,392.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{\hat{K}^{T} :}$};
% Text Node
\draw (904,412.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \mathit{d_{k} \times k}$};
% Text Node
\draw (968,366.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Value};
% Text Node
\draw (989,399.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{\hat{V}:k\times d_{v}}$};
% Text Node
\draw (847,328.6) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle \times $};
% Text Node
\draw (774,181.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Low-Rank\\Pairwise\\Similarities};
% Text Node
\draw (832,258.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle  \begin{array}{{>{\displaystyle}l}}
\mathit{\rho (S)}\\
\mathit{n \times k}
\end{array}$};
% Text Node
\draw (917,185.6) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle \times $};
% Text Node
\draw (874,99.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Output};
% Text Node
\draw (898,131.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \mathit{Y:n\times d_{v}}$};
% Text Node
\draw (43,75.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Transformer Model}};
% Text Node
\draw (373,75.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Transformer Attention};
% Text Node
\draw (733,75.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Linformer Attention};
% Text Node
\draw (600,235) node [anchor=north west][inner sep=0.75pt]   [align=center] {Reduce Complexity\\ O($N^2$) $\rightarrow$ O($N$)};
\end{tikzpicture}
}
\caption[Attention mechanism in original transformer model and Linformer model]{Comparison of the attention mechanism in original transformer model and Linformer model}
\label{fig:linformer-model}
\end{figure}

Genomics modeling for phenotype prediction such as Alzheimer's disease risk prediction can be defined as a sequence modeling for classification task. For instance, given a long sequence $X=(x_1, x_2, ..., x_n)$ as its input and the model produces a class probability $Y$ denoting the probability of the patient's risk of getting a certain phenotype. A regular attention-based method is not suitable for solving this task as the memory and computational cost of the model increase quadratically over the length of the sequence. To cope with this problem, a variant of attention-based model with linear-attention mechanism is incorporated instead of the original quadratic-attention model. Different linear-attention methods have been developed for solving long sequence NLP and computer vision tasks~\cite{kitaev2020reformer,katharopoulos2020lineartrf,shen2021efficientattn,choromanski2021performer,zaheer2020bigbird}, and in this work we extend one variant of linear-attention transformer model, i.e., Linformer \cite{wang2020linformer}, to enable long sequence genomic modeling for Alzheimer's disease prediction task. 

As shown in Figure \ref{fig:linformer-model}, Linformer reduces the complexity of attention mechanism by performing low-rank approximation to the self-attention layer of a transformer model. Mathematically, A self-attention layer accepts an input sequence $X \in \mathbb{R}^{n \times d}$ an output another sequence $X \in \mathbb{R}^{n \times d_v}$. In the original transfomer model, the input sequence $X$ is first projected into three different sequences: query $Q \in \mathbb{R}^{n \times d_k}$, key $K \in \mathbb{R}^{n \times d_k}$, and value $V \in \mathbb{R}^{n \times d_v}$ by using query projection $W^Q \in \mathbb{R}^{d \times d_k}$, key projection $W^K \in \mathbb{R}^{d \times d_k}$, and value projection $W^V \in \mathbb{R}^{d \times d_v}$, respectively. A scaled-dot product attention is then applied from the three sequences to produce the sequence $Y$. The formula for calculating the self-attention mechanism in Transformer is as follow:

\begin{align}
&Q = XW^Q, K = XW^K, V = XW^V\\
&Y=\textnormal{Softmax}(\frac{QK^T}{\sqrt{d_k}}V)
\end{align}

While in Linformer model, after $X$ is projected to $Q$, $K$, and $V$, another projection from $K \in \mathbb{R}^{n \times d_k}$ and $V \in \mathbb{R}^{n \times d_v}$ with $W^{\hat{K}} \in \mathbb{R}^{k \times n}$ and $W^{\hat{V}} \in \mathbb{R}^{k \times n}$, respectively. The projection produces a low-rank key sequence $\hat{K} \in \mathbb{R}^{k \times d_k}$ and a low-rank value sequence $\hat{V} \in \mathbb{R}^{k \times d_v}$. The complete formula for calculating the self-attention mechanism in Linformer is as follow: 

\begin{align}
&Q = XW^Q, K = XW^K, V = XW^V\\
&\hat{K} = W^{\hat{K}}K, \hat{V} = W^{\hat{V}}V\\
&Y=\textnormal{Softmax}(\frac{Q\hat{K}^T}{\sqrt{d_k}}\hat{V})
\end{align}

The additional projection steps reduce the space and time complexity of computing $Y$ from O($n^2$) to O($nk$) which can also be written as O($n$) as $k$ is a constant. If we choose the rank $k$ to be very low $k<<n$, the Linformer model could get a huge reduction in terms of both computation time and memory usage.

\section{Experimental Setup}

We conduct our experiment for Alzheimer's disease risk prediction on Chinese Cohort by comparing the effectiveness of different diploid sequence representations, 1) as a set of two haplotype sequence and 2) as a diplotype sequence. The following sections, we describe the SentencePiece training for both haplotype and diplotype tokens, the pre-training phase of our linear attention-based model, and the fine-tuning and evaluation of our models.

\subsection{Dataset Construction}

We construct a dataset of genome sequence for predicting a specific disease called late-onset Alzheimer's disease (LOAD) \cite{rabinovici2019load} on Chinese Cohort. We collect the sequencing data from 678 Hong Kong elderly with minimum age of 65. The subjects are diagnosed for any dementia related issue through Montreal Cognitive Assessment (MoCA) test \cite{nasreddine2005moca}. The score is adjusted according to the demography information, i.e., age, gender, and education year of the subject and final diagnosis is made by medical professional to decide whether the subject has cognitive impairment. From the 678 subjects, we filter out subjects with mild cognitive impairment (MCI) and other types of dementia that is not related to Alzheimer's Disease. After the filtering, we end up with 626 subjects with 386 subjects labelled as Alzheimer's disease carrier (AD) and 240 subjects labelled as non-carrier (NC). It is also worth noting that AD diagnosis through memory test is not always accurate \cite{cecato2011mocaperf} and currently, a definite AD diagnosis can only be possible through post-mortem diagnosis \cite{deture2019neuropathological}.

We collect genome sequence information from the APOE region~\cite{zhou2019apoe} located in chromosome 19 for each subject. The sequencing is done by using Ilumina platform with read depth of 5 and read length of 150. We align the sequence data with bamtools~\cite{barnett2011bamtools} using hg19 reference genome~\cite{church2011hg19} to align the sequence data. For generating diplotype, we use pysam v0.15.4 and samtools v1.7 \cite{li2009samtools} to generate the profile for each position from the aligned read data and taking top-2 values from the profile to form the diplotype. For generating two haplotypes from diploid chromosome sequence, we generate the variant calling data with Genome Analysis Tool Kit (GATK) HaplotypeCaller v3.4–46-gbc02625 ~\cite{mckenna2010gatk, depristo2011gatk, auwera2013gatk-pipeline}. Variant recalibration is then applied for SNPs and INDELs using VariantRecalibrator with truth sensitivity thresholds of 90\% and 99.9\% for INDELs and SNPs, respectively. Variants ranked by VQSLOD score that passed the sensitivity thresholds were retained for genotyping refinement and phasing using Beagle (r1399)~\cite{browning2007beagle,browning2009beagle}. We thus reconstruct the haplotype sequence from the phased variants by filling the hg19 sequence for all the positions with no variant information. 
% The complete preprocessing pipeline for generating diplotype and haplotype is shown in Figure \ref{fig:preprocessing}.

\subsubsection{SentencePiece Training}

To train the haplotype SentencePiece tokenizer, we build a training corpus generated from the GrCh37 (hg19) human reference genome \footnote{\url{https://hgdownload.soe.ucsc.edu/goldenPath/hg19/bigZips/hg19.fa.gz}}. As our fine-tuning only focus on APOE region, we construct the training data for SentencePiece from only chromosome 19 sequence. We convert the chromosome 19 sequence into a set of sentences $\mathcal{S}$. To build the sentences $S$, we first random sample $k=50$ starting points from range 0 to 5,000 from the 5' end. From each starting point we iteratively take consecutive sequences with a random length between from minimum length $a=500$ to maximum length $b=1000$ until the sequence reach the end of the corresponding chromosome. All random samplings are taken uniformly.

For diplotype SentencePiece tokenizer, we build a training corpus generated from the GrCh37 (hg19) human reference genome and the dbSNP154\footnote{\url{https://ftp.ncbi.nih.gov/snp/redesign/archive/b154}}. We use SNPs which are labelled \texttt{COMMON}\footnote{A \texttt{COMMON} SNP is defined as an SNP that has at least one 1000Genomes population with a minor allele of frequency (MAF) >= 1\% and for which 2 or more founders contribute to that minor allele frequency.} in the dbSNP154 to introduce mutation patterns into the training corpus. We fill the remaining position with the sequence from GrCh37 (hg19) human reference genome to generate a complete diplotype of the chromosome 19. We thus perform the same sampling method to generate the sentences $S$ from the diplotype sequence of the chromosome 19.

The sentences $S$ is then used as the training corpus for SentencePiece training. Specifically, we build two SentencePiece models, one for haplotype sequences and one for diplotype sequences. We utilize BPE tokenization to construct the vocabulary. We random sample 3,000,000 sentences to build a vocabulary of size 32000 with 5 and 66 base tokens for haplotype and diplotype vocabulary respectively. We add three additional special tokens ``[UNK]'', ``[CLS]'', and ``[SEP]'' to be used by the model in the pre-training and fine-tuning phases.

\subsubsection{Model Architecture}

For our diplotype model, we utilize 12 layers Linformer model with 12 heads, hidden size of 768, feed forward size of 3,072, drop out of 0.1, and and low-rank factor of 256. As haplotype model needs to handle two sequences for predicting Alzheimer's risk, we adjust the model size to make the computation cost equal with the diplotype sequence. For instance, we reduce the number of layer of the haplotype model into 6, while keeping all other hyperparameters unchanged.

\subsubsection{Pre-Training Phase}

Following the success of pre-training approach in many different fields such as NLP, computer vision, and speech processing, we perform pre-training to allow the model to learn the structure of a genome sequence. We use the same data as the one use for generating the SentencePiece models, but we concatenate several sentences into a single input sequence with maximum sequence length of 4,096 tokens. Similar to language model pre-training in NLP, we use a masked language modeling (MLM) objective to train our model. We use AdamW optimizer~\cite{loshchilov2018decoupled} to optimize our model with initial learning rate of $1\mathrm{e}-4$ and apply a step-wise learning rate decay with $\gamma=0.999991$. We run the pre-training of our model for 200,000 steps with a batch size of 256.

\subsubsection{Fine-Tuning and and Evaluation Details}

To evaluate the pre-trained models, we run a fine tuning process to adapt the model for Alzheimer's disease risk prediction task. For diplotype model, we feed the diplotype sequence and project the output from \texttt{[CLS]} token to get the prediction logits. For haplotype model, we feed each haplotype sequence into the model, concatenate both outputs of the \texttt{[CLS]} token, and project the concatenated vector to get the prediction logits.

We fine-tune the model for maximum 30 epochs with early stopping of 5, learning rate of $1\mathbb{e}-5$, and step-wise learning rate decay with $\gamma=0.9995$. We use cross-entropy loss and AdamW optimizer to optimize our model. We run the fine-tuning process 10 times with different stratify splitting for train, validation, and valid. We evaluate our models by calculating the AUC and F1-score from the model predictions and the phenotype label.

\section{Result and Discussion}

\subsection{Evaluation Performance}

\subsection{Effects of Pre-training}

\subsection{Effects of Extending Sequence Length}

\subsection{Benefit of SentencePiece Tokenization}

\subsection{Model Interpretability}

\section{Conclusion}

\newpage

==> chapter/sec-4-multimodal-e2e-sparse-model.tex <==
\chapter{Sparse Cross-Modal Attention for Multimodal Emotion Recognition}
\label{sec-sparse-cross-modal-attention}

Processing multimodal data often brings a huge computational burden. To avoid this problem, most existing works in multimodal processing tend to apply two phases-pipeline to reduce the computational cost. In the two phases-pipeline, the feature representations are first extracted from each modality with a feature extractor module such as hand-crafted algorithms or a pre-trained model. The extracted features are then used to train a model to fit to a certain task such as for classification or regression. However, there are several caveats from this approach. Firstly, the extracted features are fixed and cannot be further fine-tuned on different target tasks. Second, manual searching for the best performing feature extraction algorithms is required, which does not generalize or scale well for handling multiple tasks and can lead to a sub-optimal performance. On the other hand, a fully end-to-end model can alleviate these problems by allowing the feature extraction to be adjusted accordingly through learning during the training phase. Nevertheless, a fully end-to-end model carries a huge computational overhead compared to the two-phase pipeline by exhaustively processing all the data points across all modalities.

In this chapter, we propose a more efficient multimodal model called multimodal end-to-end sparse model (MESM), which reduce the computational overhead of the fully end-to-end model, while allowing end-to-end training mechanism. We introduce a sparse cross-modal attention mechanism to improve the efficiency of the model by dropping a significant amount of unimportant data points in the video and audio modalities. Our approach produces a set of the most relevant features for the task and reduce any redundant information and noisy features. Our experiment result suggests that MESM with sparse cross-modal attention can significantly reduce the computational cost while maintaining the evaluation score compared to the fully end-to-end model. The illustration of our sparse end-to-end model is shown in Figure~\ref{fig:scma-intro}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{images/chapter-4/SMMM-Highlight-Col.pdf}
    \caption[Illustration of different feature extraction methods]{An illustration of feature extraction from hand-crafted method (\textit{left}), fully end-to-end model (\textit{middle}), and sparse end-to-end model (\textit{right}). The red dots represent the keypoints extracted by hand-crafted models. The areas formed by red lines represent the regions of interest that are processed by (sparse) end-to-end models to extract the features.}
    \label{fig:scma-intro}
\end{figure}

\section{Methodology}

We define $I$ multimodal data samples as $X=\{(t_i,a_i,v_i)\}^I_{i=1}$, in which $t_i$ is a sequence of words, $a_i$ is a sequence of spectrogram chunks from the audio, and $v_i$ is a sequence of RGB image frames from the video. $Y=\{y_i\}^I_{i=1}$ denotes the annotation for each data sample.

\subsection{Multimodal End-to-end Sparse Model}

In this section we introduce our Multimodal End-to-end Sparse Model (MESM). As shown in Figure~\ref{fig:main_model}, for text modality, we use a transformer model~\cite{vaswani2017transformer} to extract the text representation. For audio and video modalities, we use CNN layers to extract low-level features from the raw inputs. To reduce the computation cost, we introduce Cross-modal sparse CNN block which consists of a sparse cross-modal attention layer and a sparse CNN layer~\cite{graham2018sparsecnn}. The features are then flattened and projected using a linear transformation and then feed to transformer layers with an additional \texttt{[CLS]} token to combine information between multiple timesteps. For each modality, we take the output vector at the \texttt{[CLS]} token, concatenate the vectors, and apply linear projection to get the final classification scores.

% Main model figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/chapter-4/main_model.pdf}
    \caption[Architecture of our Multimodal End-to-end Sparse Model (MESM)]{Architecture of our Multimodal End-to-end Sparse Model (MESM). On the left, we show the general architecture flow. In the middle and on the right, we exhibit the details of the cross-modal sparse CNN block, especially the cross-modal attention layer, which is the key to making the CNN model sparse.}
    \label{fig:main_model}
\end{figure*}

\subsubsection{Sparse Cross-modal Attention}

The sparse cross-modal attention layer accepts two inputs: a query vector $Q \in \mathbb{R}^d$ and a stack of feature maps $M \in \mathbb{R}^{C \times S \times H \times W}$, where $C,S,H,$ and $W$ are the number of channels, sequence length, height, and width, respectively. Sparse cross-modal attention calculate the feature importance from each feature in $M$ according to the query vector $Q$ and eliminates unnecessary features from $M$ based-on their importance score. The query vector $Q$ is retrieved from the output of \texttt{[CLS]} token from the text modality. Our sparse cross-modal attention can be formularized in the following steps:

\begin{align}
    M_q &= \text{tanh} ((W_mM + b_m) \oplus W_qQ) \label{eq:scma_1} \\ 
    M_i &= \text{softmax} (W_iM_q + b_i) \label{eq:scma_2} \\
    M_{ns} &= \text{Nucleus 
    Sampling } (M_i) \label{eq:scma_3} \\
    M_o &= M_{ns} \otimes M, \label{eq:scma_4}
\end{align}

where $W_m \in \mathbb{R}^{k \times C}$, $W_q \in \mathbb{R}^{k \times d}$, and $W_i \in \mathbb{R}^{k}$ are linear transformation weights, and $b_m \in \mathbb{R}^{k}$ and $b_i \in \mathbb{R}^1$ are biases, where $k$ is a pre-defined hyper-parameter, and $\oplus$ represents the broadcast addition operation of a tensor and a vector. Eq.\ref{eq:scma_1} shows the additive attention mechanism~\cite{bahdanau2015additive} from a given feature map $M$ and the query vector $Q$. In Eq.\ref{eq:scma_2}, the softmax function is applied to the spatial ($H \times W$) dimensions producing $M_i$ which is the spatial attention map of the feature map $M$ based-on the query $Q$. To eliminate the less important features from the feature map $M$, we generate a mask $M_{ns}$ by performing \textbf{nucleus sampling}~\cite{holtzman2019curious} on $M_i$ and take the top-$p$ portion of the probability mass in the attention map, with $p$ is a pre-defined hyper-parameter in the range of $[0, 1]$. We then apply the mask $M_{ns}$ to the feature map $M$ to generate the sparse feature map $M_o$ with degree of sparsity is controlled by the hyperparameter $p$.

\subsubsection{Sparse CNN}

To fasten the computation of the sparse feature map generated from the sparse cross-modal attention layer, we utilize submanifold sparse CNN~\cite{graham2018sparsecnn} after the cross-modal attention layer. It is leveraged for processing low-dimensional data which lies in a space of higher dimensionality. The submanifold sparse CNN layer only computes the convolution at the active positions which makes it more efficient to compute a sparse tensor. Theoretically, in terms of the amount of computation (FLOPs) at a single location, a standard convolution costs $z^2mn$ FLOPs, and a sparse convolution costs $amn$ FLOPs, where $z$ is the kernel size, $m$ is the number of input channels, $n$ is the number of output channels, and $a$ is the number of active points. As our sparse cross-modal attention layer remove a considerable amount of points, incorporating the sparse CNN gives a huge reduction of the computational cost.

\subsection{Fully End-to-End Multimodal Modeling} 

For a comparison with our MESM model, we build a fully end-to-end (FE2E) model which jointly optimizes the feature extraction and multimodal modelling phases. Specifically, we remove the sparse cross-modal attention step and replace the sparse CNN layers with the original CNN layers. Similar to MESM, the output of the last CNN layer is flattened and projected using a linear transformation and then feed to transformer layers for both audio and video modalities. We take the output vector at the \texttt{[CLS]} token from each modality, concatenate them into one vector, and perform a linear projection to get the final classification scores.

\section{Experimental Setup}

\subsection{Dataset Construction}

In this work we use two multimodal emotion recognition datasets: Interactive Emotional Dyadic Motion Capture (IEMOCAP)~\cite{busso2008iemocap} and CMU Multimodal Opinion Sentiment and Emotion Intensity (CMU-MOSEI)~\cite{zadeh2018multimodal}. For training an end-to-end multimodal model it requires the inputs to be raw data for the three modalities (visual, textual and acoustic), but the existing multimodal emotion recognition datasets cannot be directly applied for the end-to-end training due to the existing dataset provide no information to map the pre-extracted data back to the original multimodal data. To solve this problem, we reorganize the two datasets from the the original multimodal data in two steps: 1) align the text, visual and acoustic modalities; 2) split the aligned data into training, validation and test sets. In the following subsection, we first introduce the existing datasets, and then we will give a detailed description of how we reorganize them.

\subsubsection{IEMOCAP}

IEMOCAP~\cite{busso2008iemocap} is a multimodal emotion recognition dataset comprises of 151 videos. In each video, two professional actors conduct dyadic conversations in English. The dataset is labelled with six emotion categories: \textit{angry}, \textit{happy}, \textit{excited}, \textit{sad}, \textit{frustrated}, and \textit{neutral}. To generate the raw multimodal dataset for IEMOCAP, we first clip and realign the multimodal data per utterance from the provided text transcription file resulting in 7,380 data samples. Each data sample consists of three modalities: a text transcript, image frames sampled from the video at 30 Hz, and audio data with a sampling rate of 16 kHz. As the pre-extracted dataset from the existing work~\cite{busso2008iemocap} has no map to the original multimodal data, we create a new split for the raw multimodal dataset by randomly allocating 70\%, 10\%, and 20\% of data into the training, validation, and testing sets, respectively. The statistics of our dataset split are shown in Table~\ref{tab:iemocap-dataset-statistics}.

\begin{table}[!t]
\centering
\resizebox{0.70\textwidth}{!}{
\begin{tabular}{l|cc|ccc}
\toprule
\textbf{Label} &
\textbf{\begin{tabular}[c]{@{}c@{}}Avg. word \\ length\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}Avg. clip \\ duration (s)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Train \\ size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Valid \\ size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test \\ size\end{tabular}} \\
\midrule
Anger & 15.96 & 4.51 & 757 & 112 & 234 \\
Excited & 16.79 & 4.78 & 736 & 92 & 213 \\
Frustrated & 17.14 & 4.71 & 1298 & 180 & 371 \\
Happiness & 13.58 & 4.34 & 398 & 62 & 135 \\
Neutral & 13.08 & 3.90 & 1214 & 173 & 321 \\
Sadness & 14.82 & 5.50 & 759 & 118 & 207 \\
\bottomrule
\end{tabular}
}
\caption{Statistics of our IEMOCAP dataset split.}
\label{tab:iemocap-dataset-statistics}
\end{table}

\subsubsection{CMU-MOSEI} 

CMU-MOSEI~\cite{zadeh2018multimodal} consists 23,259 utterance-leve data samples collected from 3,837 videos with 1,000 diverse speakers. The dataset consists of six emotion categories: \textit{happy}, \textit{sad}, \textit{angry}, \textit{fearful}, \textit{disgusted}, and \textit{surprised}. To create the raw multimodal dataset for CMU-MOSEI, we first generate the aligned utterance-level data from the publicly accesible raw CMU-MOSEI data\footnote{\url{http://immortal.multicomp.cs.cmu.edu/raw_datasets/processed_data/cmu-mosei/seq_length_20/}}. Out of 23,259 samples, we filter out samples with invalid alignment data which results in 20,477 data samples in total. We then generate a new dataset split following the CMU-MOSEI split for the sentiment classification task \footnote{\url{http://immortal.multicomp.cs.cmu.edu/raw_datasets/processed_data/cmu-mosei/seq_length_50/mosei_senti_data_noalign.pkl}}. The statistics of the new dataset split setting are shown in Table~\ref{tab:mosei-dataset-statistics}.

\begin{table}[!t]
\centering
\resizebox{0.70\textwidth}{!}{
\begin{tabular}{l|cc|ccc}
\toprule
\textbf{Label} &
\textbf{\begin{tabular}[c]{@{}c@{}}Avg. word \\ length\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}Avg. clip \\ duration (s)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Train \\ size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Valid \\ size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test \\ size\end{tabular}} \\
\midrule
Anger & 7.75 & 23.24 & 3267 & 318 & 1015 \\
Disgust & 7.57 & 23.54 & 2738 & 273 & 744 \\
Fear & 10.04 & 28.82 & 1263 & 169 & 371 \\
Happiness & 8.14 & 24.12 & 7587 & 945 & 2220 \\
Sadness & 8.12 & 24.07 & 4026 & 509 & 1066 \\
Surprise & 8.40 & 25.95 & 1465 & 197 & 393 \\
\bottomrule
\end{tabular}
}
\caption{Statistics of our CMU-MOSEI dataset split.}
\label{tab:mosei-dataset-statistics}
\end{table}

\subsection{Hyperparameters}

Following VGG network~\cite{simonyan2014very}, we use a total of 11 CNN layers (including sparse CNN layers) and 4 maximum pooling layers for both MESM and FE2E models. For text modality, we follow the ``albert-base-v2'' configuration\footnote{\url{https://huggingface.co/albert-base-v2/blob/main/config.json}} and initialize the transformer model with the pre-trained model weight\footnote{\url{https://huggingface.co/albert-base-v2/blob/main/pytorch_model.bin}} of the corresponding configuration.

\subsection{Baselines}
Aside of the FE2E model, we add additional two-phase pipeline baselines for each dataset. In the following subsections, we describe the hand-crafted features and the models used to perform the two-phase pipeline.

\subsubsection{Feature Extraction} 
For each modality, we extract similar features to the feature set extracted in the previous works~\cite{zadeh2018multimodal,tsai2018learning,tsai2019multimodal,rahman2020integrating}.For text data, we use the pre-trained GloVe~\citep{pennington2014glove} embeddings (glove.840B.300d\footnote{\url{https://nlp.stanford.edu/projects/glove/}}).
For the visual data, we extract 35 facial action units (FAUs) using the OpenFace library\footnote{\url{https://github.com/TadasBaltrusaitis/OpenFace}}~\cite{tadas2015openface,baltrusaitis2018openface} which capture the movement of facial muscles~\citep{ekman1980facial} from the image frames in the video. For the acoustic data, we extract 142 dimension features consisting of 12 dimension bark band energy (BBE) features, 22 dimension mel-frequency cepstral coefficient (MFCC) features, and 108 statistical features from 18 phonological classes. We extract the audio features per 400 ms time frame using the DisVoice library\footnote{\url{https://github.com/jcvasquezc/DisVoice}}~\citep{vsquez2018articulation,vsquez2019phonet}. 

\subsubsection{Baseline Model} 

We incorporate four baseline models with two-phase pipeline approach: 1) late fusion LSTM (LF-LSTM) model, 2) late fusion Transformer (LF-TRANS) model, 3) Emotion Embeddings (EmoEmbs) model~\cite{Dai2020ModalityTransferableEE}, and 4) Multimodal Transformer (MulT) model~\cite{tsai2019multimodal}. The model utilized the extracted hand-crafted features explained in the previous subsection as the input and output the predicted emotion categories.

\subsection{Training and Evaluation Details}

In the training phase, we use the Adam optimizer~\cite{kingma2015adam} and binary cross-entropy loss to train all the models. In addition, we upscaled the loss for the positive samples by the ratio of the positive and negative samples to mitigate the imbalance label. We perform additional preprocessing for the text, video, and audio modalities. For the audio modality, we use mel-spectrograms with a window size of 25 ms and stride of 12.5 ms and then chunk the spectrograms per 400 ms time window. For video modality, in order to align with the two-phase baselines which extract visual features from human faces, we use a MTCNN~\cite{zhang2016mtcnn} model to get the image of the face from each of the image frames.

In the evaluation phase, following prior works~\cite{tsai2018learning,wang2019words,tsai2019multimodal,Dai2020ModalityTransferableEE}, we use the accuracy and F1-score to evaluate the models on the IEMOCAP dataset. While for CMU-MOSEI, following the existing works~\cite{zadeh2018multimodal,akhtar2019multi,Dai2020ModalityTransferableEE,tong2017combating}, we use the binary F1 and weighted accuracy (WAcc) to evaluate the model performance.

\section{Result and Discussion}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|cccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FLOPs\\ ($\times 10^9$) \end{tabular}}} & \multicolumn{2}{c}{\textbf{Angry}} & \multicolumn{2}{c}{\textbf{Excited}} & \multicolumn{2}{c}{\textbf{Frustrated}} & \multicolumn{2}{c}{\textbf{Happy}} & \multicolumn{2}{c}{\textbf{Neutral}} & \multicolumn{2}{c}{\textbf{Sad}} & \multicolumn{2}{c}{\textbf{Average}} \\
 &  & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 \\ %\hline
\midrule
\textbf{Two-phase pipeline} \\
\midrule
LF-LSTM & - & 71.2 & 49.4 & 79.3 & 57.2 & 68.2 & 51.5 & 67.2 & 37.6 & 66.5 & 47.0 & 78.2 & 54.0 & 71.8 & 49.5 \\
LF-TRANS & - & 81.9 & 50.7 & 85.3 & 57.3 & 60.5 & 49.3 & 85.2 & 37.6 & 72.4 & 49.7 & 87.4 & 57.4 & 78.8 & 50.3 \\
EmoEmbs$^\dagger$ & - & 65.9 & 48.9 & 73.5 & 58.3 & 68.5 & 52.0 & 69.6 & 38.3 & 73.6 & 48.7 & 80.8 & 53.0 & 72.0 & 49.8 \\
MulT$^\dagger$ & - & 77.9 & 60.7 & 76.9 & 58.0 & 72.4 & 57.0 & 80.0 & 46.8 & 74.9 & 53.7 & 83.5 & 65.4 & 77.6 & 56.9 \\
\midrule
\textbf{End-to-end} \\
\midrule
FE2E & 8.65 & \textbf{88.7} & \textbf{63.9} & \textbf{89.1} & \textbf{61.9} & 71.2 & 57.8 & \textbf{90.0} & 44.8 & \textbf{79.1} & \textbf{58.4} & \textbf{89.1} & \textbf{65.7} & \textbf{84.5} & \textbf{58.8} \\
MESM ($p=0.7$) & \textbf{5.18} & 88.2 & 62.8 & 88.3 & 61.2 & \textbf{74.9} & \textbf{58.4} & 89.5 & \textbf{47.3} & 77.0 & 52.0 & 88.6 & 62.2 & \textbf{84.4} & 57.4 \\ 
\bottomrule
\end{tabular}
}
\caption[Experiment results on the IEMOCAP dataset]{The results on the IEMOCAP dataset. FLOPs is the number of floating point operations per second. We report the accuracy (Acc.) and the F1-score on six emotion categories: \textit{angry}, \textit{excited}, \textit{frustrated}, \textit{happy}, \textit{neutral} and \textit{sad}. We re-run the models marked by $^\dagger$, as we use two more categories and the split is different.}
\label{tab:iemocap}
\end{table*}


\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|cccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FLOPs\\ ($\times 10^9$) \end{tabular}}} & \multicolumn{2}{c}{\textbf{Angry}} & \multicolumn{2}{c}{\textbf{Disgusted}} & \multicolumn{2}{c}{\textbf{Fear}} & \multicolumn{2}{c}{\textbf{Happy}} & \multicolumn{2}{c}{\textbf{Sad}} & \multicolumn{2}{c}{\textbf{Surprised}} & \multicolumn{2}{c}{\textbf{Average}} \\
 &  & WAcc. & F1 & WAcc. & F1 & WAcc. & F1 & WAcc. & F1 & WAcc. & F1 & WAcc. & F1 & WAcc. & F1 \\ %\hline
\midrule
\textbf{Two-phase pipeline} \\
\midrule
LF-LSTM & - & 64.5 & 47.1 & 70.5 & 49.8 & 61.7 & 22.2 & 61.3 & 73.2 & 63.4 & 47.2 & 57.1 & 20.6 & 63.1 & 43.3 \\
LF-TRANS & - & 65.3 & 47.7 & 74.4 & 51.9 & 62.1 & 24.0 & 60.6 & 72.9 & 60.1 & 45.5 & 62.1 & 24.2 & 64.1 & 44.4 \\
EmoEmbs$^\dagger$ & - & 66.8 & 49.4 & 69.6 & 48.7 & 63.8 & 23.4 & 61.2 & 71.9 & 60.5 & 47.5 & 63.3 & 24.0 & 64.2 & 44.2 \\
MulT$^\dagger$ & - & 64.9 & 47.5 & 71.6 & 49.3 & 62.9 & 25.3 & \textbf{67.2} & \textbf{75.4} & 64.0 & 48.3 & 61.4 & 25.6 & 65.4 & 45.2 \\
\midrule
\textbf{End-to-end} \\
\midrule
FE2E & 8.65 &\textbf{67.0} & \textbf{49.6} & \textbf{77.7} & \textbf{57.1} & 63.8 & 26.8 & 65.4 & 72.6 & \textbf{65.2} & \textbf{49.0} & \textbf{66.7} & \textbf{29.1} & \textbf{67.6} & \textbf{47.4} \\
MESM (0.5) & \textbf{4.34} & 66.8 & 49.3 & 75.6 & 56.4 & \textbf{65.8} & \textbf{28.9} & 64.1 & 72.3 & 63.0 & 46.6 & 65.7 & 27.2 & 66.8 & 46.8 \\ 
\bottomrule
\end{tabular}
}
\caption[Experiment results on the CMU-MOSEI dataset]{Experiment results on the CMU-MOSEI dataset. WAcc stands for weighted accuracy. We report the accuracy and the F1-score on six emotion categories: \textit{angry}, \textit{disgusted}, \textit{fear}, \textit{happy}, \textit{sad} and \textit{surprised}. We re-run the models marked by $^\dagger$, as the data we use is unaligned along the sequence length dimension and the split is different.}
\label{tab:mosei}
\end{table*}

\subsection{Evaluation Performance}

As shown in Table~\ref{tab:iemocap}, all end-to-end models surpass all of the two-phase pipeline approaches by a large margin in all evaluation metrics. This shows the superiority of the end-to-end model over the two-phase pipeline approach. Furthermore, although with only around $\sim$60\% of the FLOPs, MESM achieves comparable results with the FE2E model. This shows the effectiveness of sparse cross-modal attention mechanism to reduce the computational cost of an end-to-end multimodal model. We also observe similar trends on the CMU-MOSEI dataset as shown in Table~\ref{tab:mosei}.


\subsection{Effects of Nucleus Sampling} \label{ns}

To further analyze the performance and efficiency trade-off of the Nucleus Sampling on the MESM, we perform more experiments with different top-p values ranging from 0 to 1, with a step of 0.1. As shown in Figure~\ref{fig:ns}, the amount of computation is reduced consistently with the decrease of the top-p values. With top-p less than 0.5 there is a clear performance drop, which suggests some of the useful information for recognizing the emotion is excluded. Interestingly, with a top-p value from greater or equal to 0.5, there is no noticeable drop in the evaluation performance. This fact suggest that our MESM can achieve halve the FLOPs without hurting the performance of the end-to-end model.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.6\linewidth]{images/chapter-4/merge_perf.pdf}
  \caption[Speed vs Performance with different Nucleus Sampling top-p values]{The trend line of the \textbf{Top:} Weighted Accuracy and \textbf{Bottom:} FLOPs (x$10^9$)) of the MESM with different top-p values used in the Nucleus Sampling. \includegraphics[height=\fontcharht\font`\B]{images/chapter-4/yellow.png} represents performance of MESM, while \includegraphics[height=\fontcharht\font`\B]{images/chapter-4/red.png} represents performance of the FE2E model}

\label{fig:ns}
\end{figure}

% In Section~\ref{ns}, we conduct a more detailed discussion of the effects of the top-p values. 
\subsection{Case Study}

% Case study figure
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/chapter-4/case_study_new.pdf}
    \caption[Case study of sparse cross-modal attention on the visual modality]{Case study of sparse cross-modal attention on the visual modality on six emotion categories in CMU-MOSEI (happy, sad, angry, surprised, fear, disgusted). From left to right, we show the original image and the Nucleus Sampling ($p=0.6$) result over points in each attention layer. Red regions represent the points that are computed for the next layer.}
    \label{fig:case_study}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/chapter-4/audio_study.pdf}
    \caption[Case study of sparse cross-modal attention on the acoustic modality]{Case study of sparse cross-modal attention on the acoustic modality. We only show the highest 10\% value of mel-spectrogram in each image. From left to right, we show the original image and the Nucleus Sampling ($p=0.6$) results over points in each attention layer. Red regions represent the active points that will go to the next sparse CNN layer.}
    \label{fig:audio_case_study}
\end{figure}

To get further understanding and insights from our MESM, as shown in Figure~\ref{fig:case_study}, we visualize the attention maps of our sparse cross-modal attention mechanism on the six  emotions categories in CMU-MOSEI dataset: happy, sad, angry, surprised, fear, and disgusted.

In general, the sparse cross-modal attention removes most of the region with uniform color and maintaining most of the edge features. In most cases, MESM attends to several regions of interest that are related to the facial action coding system (FACS)~\citep{ekman1997face} such as the mouth, eyes, eyebrows, and facial muscles between the mouth and the eyes. 
We further verify our method by comparing the regions that our model captures with the mapping of FACS to human emotion categories~\cite{basori2016facial,ahn2017insideout}. According to FACS to human emotion mapping, the emotion \textit{happy} is highly influenced by raising of the lip on both ends, \textit{Angry} emotion is shown by a narrowed gap between the eyes and thinned lips, while the \textit{sad} emotion is signaled by a lowered lip on both ends and downward movement of the eyelids. \textit{surprised} emotion is indicated with raising of the eyebrows and eyelids along with an open mouth, while the emotion \textit{Fear} is expressed by an open mouth with the ends of the lips slightly moving toward the cheeks, and the emotion \textit{disgusted} is determined by wrinkles near the nose area and movement of the upper lip region

According to our attention analysis on visual modality shown in Figure~\ref{fig:case_study}, our MESM can capture most of the correct FACS regions that are related to the six emotion categories. For instance, on the emotion \textit{angry}, the sparse cross-modal attention can retrieve the features from the lip region quite well and for \textit{surprised} emotion, the eyelids and mouth regions can be perfectly captured by MESM, although the model fails to consider the eyebrow regions. 
We further perform similar analysis for the acoustic modality as shown in Figure~\ref{fig:audio_case_study}. Although there is no prior work mentioning specific acoustic patterns for emotion categories, but in general, our MESM filter out the regions with low spectrum values in the early attention layer, and further remove some more features with high spectrum values after going through more sparse cross-modal attention layers.

\begin{table}[!ht]
\centering
\resizebox{0.52\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Mods.} & \textbf{Avg. Acc} & \textbf{Avg. F1} \\ \midrule
\multirow{7}{*}{FE2E} & TAV & 84.5 & 58.5 \\
 & TA & 83.7 & 54.0 \\
 & TV & 82.8 & 55.7 \\
 & VA & 81.2 & 54.4 \\
 & T & 80.8 & 50.0 \\
 & A & 73.3 & 44.9 \\
 & V & 78.2 & 49.8 \\ \midrule
\multirow{3}{*}{MESM} & TAV & 84.4 & 57.3 \\
 & TA & 83.6 & 56.7 \\
 & TV & 82.1 & 56.0 \\ \bottomrule
\end{tabular}
}
\caption[Ablation study of FE2E and MESM]{Results of the ablation study of our fully end-to-end model (FE2E) and multimodal end-to-end sparse model (MESM) on the IEMOCAP dataset. In the Mods. (modalities) column, the T/A/V indicates the existence of the textual (T), acoustic (A), and visual (V) modalities.}
\label{tab:ablation}
\end{table}

\section{Ablation Study}

We further conduct an ablation study to investigate how the models perform when one or more modalities are absent. We show our ablation results in Table~\ref{tab:ablation}. Similar to previous works\cite{tsai2019multimodal,wang2017select,akhtar2019multi}, we observe that having more modalities leads to a better model performance. The models trained with all modalities result in the best performance for both FE2E and MESM. According to our ablation, text modality plays more important role in emotion recognition task compared to the other two modalities. This phenomenon validates that using textual (T) modality to select the important acoustic (A) and visual (V) in our sparse cross-modal attention mechanism is a reasonable choice.

\section{Conclusion}

In this chapter, we first contrast the three different approaches to accomplish multimodal emotion recognition tasks: 1) two-phase pipeline, 2) fully end-to-end (FE2E) model, and 3) multimodal end-to-end sparse model (MESM). Additionally, we reorganize two existing datasets, IEMOCAP and CMU-MOSEI to enable fully end-to-end training. Our empirical results demonstrate that the end-to-end model has an advantage in feature learning and compared to the two-phase pipeline approach. Furthermore, with the sparse cross-modal attention mechanism in MESM, we can reduce the computational cost  up to around $\sim$50\% in the multimodal end-to-end model, while maintaining its performance.

Our sparse cross-modal attention can also improve the interpretability of the model on video and audio modalities, by visualizing the sparse attention maps on both visual and acoustic data. Our case study validates that sparse cross-modal attention can select important features based on the mapping of facial action coding system (FACS) for different emotion categories. Lastly, our ablation study further validates the empirical analysis in the prior works\cite{tsai2019multimodal,akhtar2019multi,wang2017select}: 1) textual modality plays more important role in multimodal emotion recognition task and 2) using more modalities results in higher evaluation performance.

\newpage

==> chapter/sec-abstract-new.tex <==
\begin{abstract}

% In this thesis, we improve the computation and memory efficiency of the recently renowned transformer models with low-rank approximation approach. We propose two low-rank variant: Low-Rank Transformer which is especially effective for handling dynamic-length short-sequence data and further extend to Low-Rank Linformer which is more effective for handling static-length long-sequence data.

% Recent developments in transformer models tend to increase the model's size significantly and ends up with a much larger model. Although it leads to a better and more accurate prediction, the resulting model becomes even more inefficient and costly, as it requires weeks of training with a huge amount of GPU resources. In the light of this inefficiency problem, in this thesis, we improve the computation and memory efficiency of the recently renowned transformer models with low-rank approximation approach. We propose a low-rank transformer model called Low-Rank Transformer. We  Based on our analysis, Low-Rank Transformer model is suitable for improving both the time and memory efficiency in processing dynamic-length short-sequence ($\leq512$) data, while Low-Rank Linformer model is suitable for improving the efficiency in processing static-length long-sequence ($\geq512$) data. Additionally, we also show that our Low-Rank Transformer is more suitable for on-device deployment compared to the original Transformer and Linformer models, as it significantly reduces the model size as the rank decreases.

Recent methods in the efficient transformer models focus on solving long-sequence problem, while it often neglects the inefficiency problem in the short-sequence regime. In light of this limitation, in this thesis, we improve the computation and memory efficiency of the recently renowned transformer models with low-rank approximation approach for handling the short-sequence data. We propose a low-rank transformer model called Low-Rank Transformer. We compare our proposed model with the other low-rank efficient transformer model, Linformer. Based on our analysis, Low-Rank Transformer model is suitable for improving both the time and memory efficiency in processing dynamic-length short-sequence ($\leq512$) data, while Linformer model is suitable for improving the efficiency in processing static-length long-sequence ($\geq512$) data. Additionally, we also show that our Low-Rank Transformer is more suitable for on-device deployment compared to the original Transformer and Linformer models, as it significantly reduces the model size as the rank decreases.

We show the effectiveness of our Low-Rank Transformer on speech recognition task. Our result suggest that our Low-Rank Transfomer model can significantly reduce the computational time and memory usage of a speech recognition task. We apply matrix factorization on the model's parameters which can halve the size of the model and increase the speed by up to 1.35x in the GPU and 1.25x in the CPU while maintaining the performance of the model compared to the non-factorized transformer model. Our finding suggests that speech recognition models tend to be over-parameterized and our Low-Rank Tranformer method can help to mitigate the over-parameterization problem, yielding a more efficient model with a better generalization.

% We further introduce Low-Rank Linformer which combine the advantages from Low-Rank Transformer and Linformer model. Our Low-Rank Linformer can be efficient in processing short-sequence and further improve the efficiency for long-sequence data. We compare our Low-Rank Linformer model against the normal Linformer model on audio emotion classification task. Our result suggest that our Low-Rank Linformer model can further reduce the computational time and memory usage of Linformer model. Our Low-Rank Linformer model halve the size of the Linformer model, increase the speed by up to 2.00x, and even improve the performance of the model compared to the original Linformer model.

% In this thesis, we improve the computation and memory efficiency of the recently renowned transformer models with low-rank approximation approach. We propose two low-rank variant: Low-Rank Transformer which is especially effective for handling dynamic-length short-sequence data and Low-Rank Linformer which is effective for handling static-length long-sequence data.

% This computationally hungry model also incurs a substantial cost to the environment and even reaches an alarming level of carbon footprint~\cite{strubell2019energy}. Some of these models are so massive that it is even impossible to run the model in real-time with a single GPU device. 


% Recent developments in transformer models tend to increase the model's size significantly and ends up with a much larger model. Although it leads to a better and more accurate prediction, the resulting model becomes even more costly, as it requires weeks of training with a huge amount of GPU resources. This computationally hungry model also incurs a substantial cost to the environment and even reaches an alarming level of carbon footprint~\cite{strubell2019energy}. Some of these models are so massive that it is even impossible to run the model in real-time with a single GPU device. 

% we compare LRT to another l. Based on our analysis, Low-Rank Transformer model is suitable for improving both the time and memory efficiency in processing short-sequence ($\leq512$) input data, while Linformer model is suitable for improving the efficiency in processing long-sequence input data ($\geq512$). Additionally, we also show that Low-Rank Transformer is more suitable for on-device deployment, as it significantly reduces the model size as the rank decreases.

% Secondly, we present a sparse cross-modal attention mechanism for a multimodal emotion recognition model. The sparse cross-modal attention mechanism learns to remove noisy features from the video and audio modalities by using the information from the text modality, producing a smaller and more robust feature set. Our proposed model successfully reduces the FLOPS of our model by around 60\% without any considerable degradation in the evaluation performance. Our finding suggests that multimodal data consists of huge noise and our sparse-attention mechanism can eliminate these noisy features, yielding a significant speedup in terms of the computation time of the model.

% Lastly, we show the possibility of applying another low-rank model, Linformer, to a genomics study for Alzheimer's disease risk prediction. We apply the sequence modeling technique with transformer models to predict Alzheimer's disease in the Chinese cohort. We represent the problem as a long sequence prediction problem. Specifically, as the average length of a human gene is quite long ($\sim$24,000 nucleotides long), we utilize a linear-attention mechanism that enables us to process the whole sequence in an end-to-end manner. Our model is able to capture long sequence by up to  $\sim$35,000 nucleotides long and we further show that our model can boost the evaluation performance by up to $\sim$5\% AUC compared to the existing FDA-approved risk scoring model and other deep learning variants. Additionally, we show that tokenization technique can also provide a huge computation and memory efficiency by chunking the sequence which reduces the overall sequence length to be processed by the model.

\end{abstract}
